Robust Partially-Compressed Least-Squares

Randomized matrix compression techniques, such as the Johnson-Lindenstrauss transform, have emerged as an effective and practical way for solving large-scale problems efficiently. With a focus on computational efficiency, however, forsaking solutions quality and accuracy becomes the trade-off. In this paper, we investigate compressed least-squares problems and propose new models and algorithms that address the issue of error and noise introduced by compression. While maintaining computational efficiency, our models provide robust solutions that are more accurate--relative to solutions of uncompressed least-squares--than those of classical compressed variants. We introduce tools from robust optimization together with a form of partial compression to improve the error-time trade-offs of compressed least-squares solvers. We develop an efficient solution algorithm for our Robust Partially-Compressed (RPC) model based on a reduction to a one-dimensional search. We also derive the first approximation error bounds for Partially-Compressed least-squares solutions. Empirical results comparing numerous alternatives suggest that robust and partially compressed solutions are effectively insulated against aggressive randomized transforms.

==> guaranteesForPCLS.tex <==

\section{Approximation Error Bounds for Partially-Compressed Least Squares} \ban{not sure if ``approximation error'' is the right term?}
discuss previous results from Pilanci and Wainwright and how we present corresponding results for the partial-compressed case
\subsection{Guarantees for sub-Gaussian sketches and for randomized orthogonal systems}

If we use Lemma \ref{epsilon-optimal} for partial-compressed variants of the convex program in \cite{Pilanci-Wainwright}, do we have improved variants of Theorem 1 and Theorem 2? 

\begin{defn}[$\epsilon$-optimal solution]
We say that a solution $\hat{x}$ is $\epsilon$-optimal if it satisfies
\begin{equation} \label{eq:epsilon-optimal}
\frac{\|A(\hat{x} - x^*)\|}{\|A x^*\|} \leq \epsilon, \quad \epsilon \in (0,1)
\end{equation}
where $x^*$ is an optimal solution. 
\end{defn}

\begin{thm}[Approximation Guarantee] \label{thm:approx-error-bounds}
Given a sketching matrix $\Phi \in \R^{m \times N}$, and universal constants $c_0, c_1, c_2$, the sketched solution $x_{PCLS}$ \eqref{eq:x-PCLS} is $\epsilon$-optimal \eqref{eq:epsilon-optimal} with probability at least $1 - c_1\exp(-c_2\,m\,\epsilon^2)$, for any tolerance parameter $\epsilon \in (0,1)$,  \underline{when} the sketch or compression size $m$ is bounded below by
\begin{itemize}
\item[(i)]  $m > c_0 \frac{rank(A)}{\epsilon^2}$, if $\Phi$ is a sub-Gaussian sketch 
\item[(ii)] $m > c'_0 \frac{rank(A)}{\epsilon^2}\log^4(n)$, if $\Phi$ is a randomized orthogonal systems (ROS) sketch
\end{itemize}
\end{thm}

To obtain these results, we first have to prove the following lemma which shows that the partial-compressed solution $x_\PCLS$ is $\epsilon$-optimal for sub-Gaussian and ROS sketches.

\begin{lem}\label{lem:epsilon-optimal-guarantees}
For any sketch $\Phi \in \R^{m \times N}$ that is either sub-Gaussian or (ROS), the partial-compressed solution $X_\PCLS$ \eqref{eq:x-PCLS} is $\epsilon$-optimal \eqref{eq:epsilon-optimal} relative to the optimal solution $x_\LS$ \eqref{eq:x-LS} of the original high-dimensional system.
\end{lem}
\begin{proof}
From the optimality of $x_\PCLS$ and feasibility of $x_\LS$ to the partial-compressed least squares problem \eqref{eq:PCLS}, we have:
\begin{equation}
\|\Phi A x_\PCLS\|^2 \leq \|\Phi A x_\LS \|^2 + 2 \langle A\,(x_\PCLS - x_\LS), y\rangle
\end{equation}
where $\langle\cdot,\cdot\rangle$ denotes the inner product. Along with
\[ \|\Phi A\,(x_\PCLS - x_\LS)\|^2 = \|\Phi A x_\PCLS\|^2 + \|\Phi A x_\LS \|^2 -2 \langle\Phi A x_\PCLS, \Phi A x_\LS\rangle \]
we can show that
\begin{flalign*}
\frac{1}{2} \|\Phi A\,(x_\PCLS - x_\LS)\|^2 &\leq \|\Phi A x_\LS \|^2 + \langle A\,(x_\PCLS - x_\LS), y\rangle - \langle\Phi A x_\PCLS, \Phi A x_\LS\rangle\\
&\leq \langle A\,(x_\PCLS - x_\LS), y\rangle - \langle\Phi A \,(x_\PCLS - x_\LS), \Phi A x_\LS\rangle\\
&\leq \left|\langle A\,(x_\PCLS - x_\LS), (\Phi^T\Phi + I)A x_\LS \rangle \right|
\end{flalign*}
where the last two inequalities follow by adding and subtracting terms and noting that $\langle A\,(x_\PCLS - x_\LS), (A x_\LS - y) \rangle \geq 0$ from the optimality of $x_\LS$ \eqref{eq:x-LS}. Normalizing both sides of the last inequality appropriately, we obtain:

\[\frac{1}{2} \underbrace{\frac{\|\Phi A\,(x_\PCLS - x_\LS)\|^2}{\|A\,(x_\PCLS - x_\LS)\|^2}}_\text{$U_1$}\|A\,(x_\PCLS - x_\LS)\|  \leq \|A x_\LS \| \underbrace{\left|\langle \frac{A\,(x_\PCLS - x_\LS)}{\|A\,(x_\PCLS - x_\LS)\|}, (\Phi^T\Phi - I)\frac{A x_\LS}{\|A x_\LS \|} \rangle \right|}_\text{$U_2$} \]
to complete the proof, we need to show that $2\,\frac{U_2}{U_1}$ is bounded above by $\epsilon \in (0,1)$ for both the sub-Gaussian sketch and the ROS sketch. To do so, we rely on results in \cite{Pilanci-Wainwright}; the bound for sub-Gaussian sketches is implied by Lemma~2 and Lemma~3 and for ROS sketches by Lemma~4 and Lemma~5.
\end{proof}
The proof of Theorem~\ref{thm:approx-error-bounds} follows immediately from Corollary~2 in \cite{Pilanci-Wainwright} and from applying Lemma~\ref{lem:epsilon-optimal-guarantees} above.
\paragraph{Remark.} 

